Wisdom of the Ensemble: Improving Consistency of Deep Learning Models

Deep learning classifiers are assisting humans in making decisions and hence the user's trust in these models is of paramount importance. Trust is often a function of constant behavior. From an AI model perspective it means given the same input the user would expect the same output, especially for correct outputs, or in other words consistently correct outputs. This paper studies a model behavior in the context of periodic retraining of deployed models where the outputs from successive generations of the models might not agree on the correct labels assigned to the same input. We formally define consistency and correct-consistency of a learning model. We prove that consistency and correct-consistency of an ensemble learner is not less than the average consistency and correct-consistency of individual learners and correct-consistency can be improved with a probability by combining learners with accuracy not less than the average accuracy of ensemble component learners. To validate the theory using three datasets and two state-of-the-art deep learning classifiers we also propose an efficient dynamic snapshot ensemble method and demonstrate its value.

==> sections/ccsxml.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010257.10010321.10010333</concept_id>
       <concept_desc>Computing methodologies~Ensemble methods</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010293.10010294</concept_id>
       <concept_desc>Computing methodologies~Neural networks</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010258.10010259.10010263</concept_id>
       <concept_desc>Computing methodologies~Supervised learning by classification</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Ensemble methods}
\ccsdesc[500]{Computing methodologies~Neural networks}
\ccsdesc[300]{Computing methodologies~Supervised learning by classification}


==> sections/thm-label.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{SmartManufacturing,Dermatologist}
\citation{Ashoori2019InAW,varshney2020mismatched}
\citation{DLLoanApproval}
\citation{crane2018questionable}
\providecommand \oddpage@label [2]{}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}\protected@file@percent }
\newlabel{sec:introduction}{{1}{1}{Introduction}{section.1}{}}
\citation{anil2018large,patil2018training,islam2017reproducibility}
\citation{lakshminarayanan2017simple,snoek2019can}
\citation{olorisade2017reproducibility,kenett2015clarifying}
\citation{islam2017reproducibility,patil2018training}
\citation{kenett2015clarifying}
\citation{anil2018large,patil2018training,islam2017reproducibility}
\citation{anil2018large}
\citation{patil2018training}
\citation{islam2017reproducibility}
\citation{ren2016ensemble}
\citation{wang2003mining,abdullah2009ensemble,cirecsan2012multi,agostinelli2013adaptive,xie2013horizontal,huang2017snapshot}
\citation{gal2016dropout,lakshminarayanan2017simple,snoek2019can}
\citation{wang2003mining}
\citation{pietruczuk2017adjust}
\citation{bonab2019less}
\citation{breiman1996bagging}
\citation{freund1996experiments}
\citation{hinton2012improving}
\citation{huang2017snapshot}
\citation{abdullah2009ensemble}
\citation{ciregan2012multi}
\citation{agostinelli2013adaptive}
\citation{lakshminarayanan2017simple}
\citation{lee2015m}
\citation{baldi2013understanding}
\citation{hinton2012improving}
\citation{gal2016dropout}
\citation{huang2017snapshot}
\citation{loshchilov2016sgdr}
\@writefile{toc}{\contentsline {section}{\numberline {2}Related work}{2}{section.2}\protected@file@percent }
\newlabel{sec:relatedwork}{{2}{2}{Related work}{section.2}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Problem definition}{3}{section.3}\protected@file@percent }
\newlabel{sec:problem}{{3}{3}{Problem definition}{section.3}{}}
\newlabel{def:model}{{1}{3}{}{definition.1}{}}
\newlabel{def:learner}{{2}{3}{}{definition.2}{}}
\newlabel{def:copy}{{3}{3}{}{definition.3}{}}
\newlabel{def:reproducibility}{{4}{3}{}{definition.4}{}}
\newlabel{def:acc-reproducibility}{{5}{3}{}{definition.5}{}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Why ensemble?}{3}{section.4}\protected@file@percent }
\newlabel{sec:why}{{4}{3}{Why ensemble?}{section.4}{}}
\citation{bonab2019less}
\newlabel{eq:distance}{{1}{4}{Why ensemble?}{equation.4.1}{}}
\newlabel{eq:centroid}{{2}{4}{Why ensemble?}{equation.4.2}{}}
\newlabel{theorem:averaging}{{1}{4}{}{theorem.1}{}}
\newlabel{eq:theorem}{{3}{4}{}{equation.4.3}{}}
\newlabel{theorem:averaging-1}{{2}{4}{}{theorem.2}{}}
\newlabel{eq:theorem-1}{{4}{4}{}{equation.4.4}{}}
\newlabel{theorem:acc-rep}{{3}{4}{}{theorem.3}{}}
\newlabel{eq:acc-rep}{{5}{4}{}{equation.4.5}{}}
\newlabel{corollary:ccon}{{3.1}{4}{}{corollary.3.1}{}}
\newlabel{eq:acc-rep-lemma}{{6}{4}{}{equation.4.6}{}}
\citation{lakshminarayanan2017simple}
\citation{huang2017snapshot}
\citation{huang2017snapshot}
\citation{loshchilov2016sgdr}
\@writefile{toc}{\contentsline {section}{\numberline {5}Dynamic snapshot ensemble method}{5}{section.5}\protected@file@percent }
\newlabel{sec:framework}{{5}{5}{Dynamic snapshot ensemble method}{section.5}{}}
\@writefile{loa}{\contentsline {algocf}{\numberline {1}{\ignorespaces Pseudocode of the dynamic snapshot ensemble\relax }}{5}{algocf.1}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{alg:framework}{{1}{5}{Dynamic snapshot ensemble method}{algocf.1}{}}
\citation{zhang2015text}
\citation{krizhevsky2009learning}
\citation{he2016deep}
\citation{joulin2016bag}
\citation{gal2016dropout}
\citation{huang2017snapshot}
\newlabel{subsec:prune}{{11}{6}{Dynamic snapshot ensemble method}{algocf.1}{}}
\newlabel{eq:prune}{{7}{6}{Dynamic snapshot ensemble method}{equation.5.7}{}}
\newlabel{subsec:combine}{{11}{6}{Dynamic snapshot ensemble method}{equation.5.7}{}}
\@writefile{toc}{\contentsline {section}{\numberline {6}Experimental results and analysis}{6}{section.6}\protected@file@percent }
\newlabel{sec:result}{{6}{6}{Experimental results and analysis}{section.6}{}}
\newlabel{subsec:metric}{{6}{6}{Experimental results and analysis}{section.6}{}}
\newlabel{subsec:data}{{6}{6}{Experimental results and analysis}{section.6}{}}
\newlabel{subsec:method}{{6}{6}{Experimental results and analysis}{table.caption.3}{}}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Data and Models\relax }}{7}{table.caption.3}\protected@file@percent }
\newlabel{tab:data-model}{{1}{7}{Data and Models\relax }{table.caption.3}{}}
\newlabel{subsec:setting}{{6}{7}{Experimental results and analysis}{table.caption.3}{}}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces ACC, CON, ACC-CON performance and run-time of each method. $\kappa $ is one training time from scratch using the base model and model settings. \relax }}{7}{table.caption.4}\protected@file@percent }
\newlabel{tab:result}{{2}{7}{ACC, CON, ACC-CON performance and run-time of each method. $\kappa $ is one training time from scratch using the base model and model settings. \relax }{table.caption.4}{}}
\newlabel{subsec:result}{{6}{7}{Experimental results and analysis}{table.caption.4}{}}
\citation{ren2016ensemble}
\citation{huang2017snapshot}
\newlabel{fig:m}{{1a}{8}{Subfigure 1a}{subfigure.1.1}{}}
\newlabel{sub@fig:m}{{(a)}{a}{Subfigure 1a\relax }{subfigure.1.1}{}}
\newlabel{fig:beta}{{1b}{8}{Subfigure 1b}{subfigure.1.2}{}}
\newlabel{sub@fig:beta}{{(b)}{b}{Subfigure 1b\relax }{subfigure.1.2}{}}
\newlabel{fig:N}{{1c}{8}{Subfigure 1c}{subfigure.1.3}{}}
\newlabel{sub@fig:N}{{(c)}{c}{Subfigure 1c\relax }{subfigure.1.3}{}}
\newlabel{fig:window}{{1d}{8}{Subfigure 1d}{subfigure.1.4}{}}
\newlabel{sub@fig:window}{{(d)}{d}{Subfigure 1d\relax }{subfigure.1.4}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Sensitivity analysis on CIFAR100+ResNet20 using DynSnap-cyc with AVG combination. (a) Varying ensemble size $m$ with $\beta =\beta ^*,N=10,T/N=20$. (b) Varying prune factor $\beta $ with $m=20, N=10, T/N=20$. (c) Varying snapshot number $N$ with $m=N, \beta =1, T/N=20$. (d) Varying snapshot window size $T/N$ with $m=20, \beta =1, N=10$.\relax }}{8}{figure.caption.5}\protected@file@percent }
\newlabel{fig:sensitivity}{{1}{8}{Sensitivity analysis on CIFAR100+ResNet20 using \dynens -cyc with AVG combination. (a) Varying ensemble size $m$ with $\beta =\beta ^*,N=10,T/N=20$. (b) Varying prune factor $\beta $ with $m=20, N=10, T/N=20$. (c) Varying snapshot number $N$ with $m=N, \beta =1, T/N=20$. (d) Varying snapshot window size $T/N$ with $m=20, \beta =1, N=10$.\relax }{figure.caption.5}{}}
\@writefile{lof}{\contentsline {subfigure}{\numberline{(a)}{\ignorespaces {ensemble size, $m$}}}{8}{subfigure.1.1}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(b)}{\ignorespaces {prune factor, $\beta $}}}{8}{subfigure.1.2}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(c)}{\ignorespaces {\# of snapshots, $N$}}}{8}{subfigure.1.3}\protected@file@percent }
\@writefile{lof}{\contentsline {subfigure}{\numberline{(d)}{\ignorespaces {window size, $T/N$}}}{8}{subfigure.1.4}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {7}Conclusion and future work}{8}{section.7}\protected@file@percent }
\newlabel{sec:conclusion}{{7}{8}{Conclusion and future work}{section.7}{}}
\bibstyle{acm}
\bibdata{ref}
\bibcite{DLLoanApproval}{{1}{}{{}}{{}}}
\bibcite{abdullah2009ensemble}{{2}{}{{}}{{}}}
\bibcite{abramowitz1965handbook}{{3}{}{{}}{{}}}
\bibcite{agostinelli2013adaptive}{{4}{}{{}}{{}}}
\bibcite{anil2018large}{{5}{}{{}}{{}}}
\bibcite{Ashoori2019InAW}{{6}{}{{}}{{}}}
\bibcite{baldi2013understanding}{{7}{}{{}}{{}}}
\bibcite{bonab2019less}{{8}{}{{}}{{}}}
\bibcite{breiman1996bagging}{{9}{}{{}}{{}}}
\bibcite{ciregan2012multi}{{10}{}{{}}{{}}}
\bibcite{cirecsan2012multi}{{11}{}{{}}{{}}}
\bibcite{crane2018questionable}{{12}{}{{}}{{}}}
\bibcite{Dermatologist}{{13}{}{{}}{{}}}
\bibcite{freund1996experiments}{{14}{}{{}}{{}}}
\bibcite{gal2016dropout}{{15}{}{{}}{{}}}
\bibcite{he2016deep}{{16}{}{{}}{{}}}
\@writefile{toc}{\contentsline {section}{\numberline {8}Broader impact}{9}{section.8}\protected@file@percent }
\newlabel{sec:broaderimpact}{{8}{9}{Broader impact}{section.8}{}}
\bibcite{hinton2012improving}{{17}{}{{}}{{}}}
\bibcite{huang2017snapshot}{{18}{}{{}}{{}}}
\bibcite{islam2017reproducibility}{{19}{}{{}}{{}}}
\bibcite{joulin2016bag}{{20}{}{{}}{{}}}
\bibcite{kenett2015clarifying}{{21}{}{{}}{{}}}
\bibcite{krizhevsky2009learning}{{22}{}{{}}{{}}}
\bibcite{lakshminarayanan2017simple}{{23}{}{{}}{{}}}
\bibcite{lee2015m}{{24}{}{{}}{{}}}
\bibcite{loshchilov2016sgdr}{{25}{}{{}}{{}}}
\bibcite{olorisade2017reproducibility}{{26}{}{{}}{{}}}
\bibcite{patil2018training}{{27}{}{{}}{{}}}
\bibcite{pietruczuk2017adjust}{{28}{}{{}}{{}}}
\bibcite{ren2016ensemble}{{29}{}{{}}{{}}}
\bibcite{snoek2019can}{{30}{}{{}}{{}}}
\bibcite{varshney2020mismatched}{{31}{}{{}}{{}}}
\bibcite{wang2003mining}{{32}{}{{}}{{}}}
\bibcite{SmartManufacturing}{{33}{}{{}}{{}}}
\bibcite{xie2013horizontal}{{34}{}{{}}{{}}}
\bibcite{zhang2015text}{{35}{}{{}}{{}}}
\citation{abramowitz1965handbook}
\@writefile{toc}{\contentsline {section}{\numberline {A}List of Notations}{12}{appendix.A}\protected@file@percent }
\newlabel{apx:notations}{{A}{12}{List of Notations}{appendix.A}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces Notations and their meanings\relax }}{12}{table.caption.7}\protected@file@percent }
\newlabel{tab:notation}{{3}{12}{Notations and their meanings\relax }{table.caption.7}{}}
\@writefile{toc}{\contentsline {section}{\numberline {B}Proof of Theorem\nobreakspace  {}\ref  {theorem:averaging}}{12}{appendix.B}\protected@file@percent }
\newlabel{apx:proof1}{{B}{12}{Proof of Theorem~\ref {theorem:averaging}}{appendix.B}{}}
\newlabel{eq:mink-apx}{{8}{12}{Proof of Theorem~\ref {theorem:averaging}}{equation.B.8}{}}
\newlabel{eq:substitute-mink-apx}{{9}{12}{Proof of Theorem~\ref {theorem:averaging}}{equation.B.9}{}}
\@writefile{toc}{\contentsline {section}{\numberline {C}Proof of Theorem\nobreakspace  {}\ref  {theorem:averaging-1}}{12}{appendix.C}\protected@file@percent }
\newlabel{apx:proof2}{{C}{12}{Proof of Theorem~\ref {theorem:averaging-1}}{appendix.C}{}}
\@writefile{toc}{\contentsline {section}{\numberline {D}Proof of Theorem\nobreakspace  {}\ref  {theorem:acc-rep}}{12}{appendix.D}\protected@file@percent }
\newlabel{apx:proof3}{{D}{12}{Proof of Theorem~\ref {theorem:acc-rep}}{appendix.D}{}}
\citation{bonab2019less}
\@writefile{toc}{\contentsline {section}{\numberline {E}Proof of Corollary\nobreakspace  {}\ref  {corollary:ccon}}{13}{appendix.E}\protected@file@percent }
\newlabel{apx:proof4}{{E}{13}{Proof of Corollary~\ref {corollary:ccon}}{appendix.E}{}}
\newlabel{eq:acc}{{10}{13}{Proof of Corollary~\ref {corollary:ccon}}{equation.E.10}{}}
\newlabel{eq:acc-rep-x}{{11}{13}{Proof of Corollary~\ref {corollary:ccon}}{equation.E.11}{}}
\newlabel{eq:acc-rep-y}{{12}{13}{Proof of Corollary~\ref {corollary:ccon}}{equation.E.12}{}}
\@writefile{toc}{\contentsline {section}{\numberline {F}Metrics}{13}{appendix.F}\protected@file@percent }
\newlabel{apx:metric}{{F}{13}{Metrics}{appendix.F}{}}
\newlabel{eq:abr}{{13}{13}{Metrics}{equation.F.13}{}}
\newlabel{eq:abk}{{14}{13}{Metrics}{equation.F.14}{}}
\newlabel{eq:ark}{{15}{13}{Metrics}{equation.F.15}{}}
\@writefile{toc}{\contentsline {section}{\numberline {G}Experiment design}{14}{appendix.G}\protected@file@percent }
\newlabel{apx:setting}{{G}{14}{Experiment design}{appendix.G}{}}
\@writefile{toc}{\contentsline {section}{\numberline {H}Dataset Design}{14}{appendix.H}\protected@file@percent }
\newlabel{apx:data}{{H}{14}{Dataset Design}{appendix.H}{}}
\providecommand\NAT@force@numbers{}\NAT@force@numbers
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Metrics computation in the experiments.\relax }}{15}{figure.caption.8}\protected@file@percent }
\newlabel{fig:design}{{2}{15}{Metrics computation in the experiments.\relax }{figure.caption.8}{}}
\@writefile{toc}{\contentsline {section}{\numberline {I}Additional metric results}{15}{appendix.I}\protected@file@percent }
\newlabel{apx:result}{{I}{15}{Additional metric results}{appendix.I}{}}
\@writefile{lot}{\contentsline {table}{\numberline {4}{\ignorespaces Additional consistency and accuracy results.\relax }}{15}{table.caption.9}\protected@file@percent }
\newlabel{tab:result-extend}{{4}{15}{Additional consistency and accuracy results.\relax }{table.caption.9}{}}
\@writefile{toc}{\contentsline {section}{\numberline {J}Sensitivity analysis settings}{15}{appendix.J}\protected@file@percent }
\newlabel{apx:sensitivityresult}{{J}{15}{Sensitivity analysis settings}{appendix.J}{}}

